On the Correctness of Automatic Differentiation for Neural Networks with Machine-Representable Parameters

Recent work has shown that forward- and reverse- mode automatic differentiation (AD) over the reals is almost always correct in a mathematically precise sense. However, actual programs work with machine-representable numbers (e.g., floating-point numbers), not reals. In this paper, we study the correctness of AD when the parameter space of a neural network consists solely of machine-representable numbers. In particular, we analyze two sets of parameters on which AD can be incorrect: the incorrect set on which the network is differentiable but AD does not compute its derivative, and the non-differentiable set on which the network is non-differentiable. For a neural network with bias parameters, we first prove that the incorrect set is always empty. We then prove a tight bound on the size of the non-differentiable set, which is linear in the number of non-differentiabilities in activation functions, and give a simple necessary and sufficient condition for a parameter to be in this set. We further prove that AD always computes a Clarke subderivative even on the non-differentiable set. We also extend these results to neural networks possibly without bias parameters.

==> packages.tex <==
%auto-ignore

\usepackage{cleveref} % for \cref{..}
\usepackage{subcaption} % for \begin{subfigure}
\usepackage{mathtools}
\usepackage{amsmath}
\usepackage{stmaryrd}
\usepackage{etoolbox} % for \ifstrempty
%% \usepackage{xspace} % for \xspace
\usepackage{mathbbol} % for \mathbb{abc}
\RequirePackage{paralist}
\usepackage{enumitem}
\usepackage{multirow} % for \multirow
%% \usepackage{proof} % for \infer
\usepackage{array}
%% \usepackage{nccmath} % for \medint\int
\usepackage{graphicx}
\usepackage{etoc} % for table of contents
%% \usepackage{tikz}

%\DeclareMathAlphabet{\mymathbb}{U}{BOONDOX-ds}{m}{n}

%%% theorem setting.
\AtEndPreamble{%
  %% \theoremstyle{definition} 
  \theoremstyle{acmdefinition} 
  \newtheorem{remark}[theorem]{Remark}
  \newtheorem{assumption}{Assumption}
  \newtheorem*{assumptionnon}{Assumption}
  \newtheorem{condition}{Condition}
  \newtheorem{property}{Property}
  %% \theoremstyle{plain}
  \theoremstyle{acmplain}
  \newenvironment{definition*}
                 {\pushQED{\qed}\definition}
                 {\enddefinition}  
  \newenvironment{example*}
                 {\pushQED{\qed}\example}
                 {\popQED\endremark}  
  \newenvironment{remark*}
                 {\pushQED{\qed}\remark}
                 {\popQED\endremark}  
  \newenvironment{assumption*}
                 {\pushQED{\qed}\assumption}
                 {\popQED\endremark}  
  \newenvironment{assumptionnon*}
                 {\pushQED{\qed}\assumptionnon}
                 {\endremark}  
  \newenvironment{condition*}
                 {\pushQED{\qed}\condition}
                 {\popQED\endremark}  
  \newenvironment{property*}
                 {\pushQED{\qed}\property}
                 {\popQED\endremark}  
}

%%% cref setting.
\crefname{assumption}{Assumption}{Assumptions}
\crefname{figure}{Fig{.}}{Figs{.}}%{Figures}
\crefname{table}{Table}{Tables}
\crefname{definition}{Definition}{Definitions}
\crefname{theorem}{Theorem}{Theorems}
\crefname{lemma}{Lemma}{Lemmas}
\crefname{proposition}{Proposition}{Propositions}
\crefname{corollary}{Corollary}{Corollaries}
\crefname{problem}{Problem}{Problems}
\crefname{example}{Example}{Examples}
\crefname{fact}{Fact}{Facts}
\crefname{conjecture}{Conjecture}{Conjectures}
\crefname{remark}{Remark}{Remarks}
\crefname{condition}{Condition}{Conditions}
\crefname{requirement}{Requirement}{Requirements}
\crefname{enumi}{}{}
%% \crefname{equation}{Eq.}{Eqs.}
\crefname{equation}{Eq{.}}{Eqs{.}}
%% \crefname{section}{{\S}}{{\S}}
\crefformat{section}{\S#2#1#3}
\crefmultiformat{section}{\S#2#1#3}{ and~\S#2#1#3}{, \S#2#1#3}{, and~\S#2#1#3}
\crefformat{appendix}{\S#2#1#3}
\crefmultiformat{appendix}{\S#2#1#3}{ and~\S#2#1#3}{, \S#2#1#3}{, and~\S#2#1#3}
\newcommand{\crefrangeconjunction}{--}
\newcommand{\creflastconjunction}{, and\nobreakspace}

